Using Program Synthesis and Inductive Logic Programming to solve Bongard Problems

The ability to recognise and make analogies is often used as a measure or test of human intelligence. The ability to solve Bongard problems is an example of such a test. It has also been postulated that the ability to rapidly construct novel abstractions is critical to being able to solve analogical problems. Given an image, the ability to construct a program that would generate that image is one form of abstraction, as exemplified in the Dreamcoder project. In this paper, we present a preliminary examination of whether programs constructed by Dreamcoder can be used for analogical reasoning to solve certain Bongard problems. We use Dreamcoder to discover programs that generate the images in a Bongard problem and represent each of these as a sequence of state transitions. We decorate the states using positional information in an automated manner and then encode the resulting sequence into logical facts in Prolog. We use inductive logic programming (ILP), to learn an (interpretable) theory for the abstract concept involved in an instance of a Bongard problem. Experiments on synthetically created Bongard problems for concepts such as 'above/below' and 'clockwise/counterclockwise' demonstrate that our end-to-end system can solve such problems. We study the importance and completeness of each component of our approach, highlighting its current limitations and pointing to directions for improvement in our formulation as well as in elements of any Dreamcoder-like program synthesis system used for such an approach.

==> discussion.tex <==
% THis is now part of results

% \subsection{Limitations}
% There are several limitations to the proposed system.
% \begin{enumerate}
%     \item Although our system is automated in nature, there is no end to end learning. Our system is composed of multiple different parts working in tandem. This makes our system vulnerable to assumptions of the individual modules such as the kinds of information added to states that may or may not be relevant to the final classification theory learnt by the Inductive Logic Programming Engine.
%     \item The initial problem figure has to necessarily match the output of a graphical program. In other words, neither can our system work on top of hand drawn images such as the originally proposed Bongard problems nor can it produce programs for images containing a lot to draw (such as the most of the Bongard problems in the range $90$-$100$, due to limitation of program lengths and computationally expensive search times in Dreamcoder).
%     \item Given that our system is strongly syntactic and typed in nature, it also falls prey to being very \textit{rigid}. This means that unlike human intelligence which is arguably much more fluid in nature.
% \end{enumerate}
% \subsection{Future Improvements}

% Here we suggest potential improvements that can resolve some of the limitations raised previously. 
% \begin{enumerate}
%     \item Although Dreamcoder creates a generative model that uses a convolutional neural network, it may not be the optimal way for reducing the search space. In particular, the search can use guidance signals during enumeration from the perceptual domain. With this form of guided-enumeration, the search times can be massively reduced and longer programs can be induced as well. Additionally, \todo{human drawn images, flush out the point about locations more}.
%     \item Various other forms of state decorations can be introduced. In our preliminary examination, three basic forms of decorations are added. Using a learnt program based feature extraction, a multitude of features can be introduced such as the ones in \cite{Depeweg2018SolvingBP}. \todo{Improve}
%     \item 
% \end{enumerate}

==> intro_as.tex <==

\section{indtroduction}

It has long been understood that choice of representation can make a significant difference
to the efficacy of machine-based induction. A seminal paper by Quinlan \cite{quin79} demonstrates
the increasing complexity of models constructed for a series of classification problems defined
on a chess endgame, using
a representation consisting of 25 features (called {\em properties\/} in the paper). He concludes:
``This immediat ely raises the question of whether these and other properties used in the study were appropriate.
The answer is that they were probably not; it seems likely that a chess expert could develop more pertinent
attributes \ldots If the expert does his job well the induction problem is simplified; if a non-expert
undertakes the definition of properties (as was the case here) the converse is true.''
Although Quinlan assumed the representation would be identified manually, the possibility of automatic
identification of an appropriate representation was already apparent to Amarel, 10 years earlier: ``
An understanding of the relationship between problem formulation and problem solving efficiency is
a prerequisite for the design of procedures that can automatically choose the most `appropriate'
representation of a problem (they can find a `point of view'of the problem that maximally
simplifies the process of finding a solution).'' \cite{amarel68}. In fact, by `choose' what
is probably meant is `construct', if we are to avoid kicking Feigenbaum's bottlneck down the
road from extracting models to extracting representations. 

It has also been understood that neural networks can automatically construct representations
of data \cite{something}. But
extraction and re-use of these representations for multiple tasks have become substantially more
common only recently, with the routine availability of specialised hardware. This has allowed
the construction of ``deep'' networks with several levels of functional composition (10s are now common, but 100s are also within
computational range). In principle, while a single layer of functional composition is all that is needed,
it is thought that the principal benefit of the additional layers lies in constructing representations that
are multiple levels of abstractions, allowing more efficient modelling.
There are however 3 important issues that have surfaced:
(1) Automatic construction of abstractions in this way requires a lot of data, often
	100s of 1000s of examples;
(2) The kinds of deep networks used for constructing abstractions depends on the type of data.
For example, certain kinds of networks are used for text, others for images and so on: there is
apparently no single approach for representation-learning that can automatically adjust to
the data type; and
(3) The internal representations of data are opaque to human-readibility, making it
difficult to achieve the kind of understanding identified by Amarel.

Recently, neural-based methods for the automatic synthesis of programs suggest
the possibility that some of these difficulties may be resolved by representing data.
Of particular interest are neural-based methods like Dreamcoder \cite{dream} that automatically
construct programs for generating data, given some primitive functions represented in
a symbolic form (Dreamcoder uses $\lambda$-expressions for the primitive functions).
A neural-network based search is performed to direct the hierarchical construction of
higher-level functions (abstractions) by composition of lower-level ones. Compositions are constructed
and assessed for utility in inter-leaved  phases
of generate-and-test (called ``Dream'' and ``Wake'' phases), until the neural-machinery
arrives at a small program, consisting the sequential composition of primitive- and invented functions.
The final result is some approximation to the Bayesian MAP program for generating the data
provided, assuming a prior preference for small programs. There are good reasons to
look at this form of program-synthesis as a mechanism for automated representation-learning:
(a) Empirical results with programs like Dreamcoder show that it is possible to identify
	programs with small numbers of examples (the need for large numbers of examples is
	side-stepped by an internal mechanism for generating data in the Dream phase);
(b) In principle, the symbolic language adopted for primitive functions ($\lambda$-expressions) and
	the mechanism of function composition is sufficiently expressive for constructing programs
	for data of any type; 
(c) The intermediate representations have clearly defined interpretations, based on functional
	composition. Besides human-readability, an added benefit results from automated
	induction techniques like those developed in Inductive Logic Programming (ILP),
	that can directly use these symbolic abstractions for constructing
	discriminatory models.

There are however some shortcomings. First, the Dreamcoder-like approach to program-synthesis has
only been demonstrated on very simple generative tasks of a geometric nature. Second, no general
technique for the re-use of intermediate representations by techniques like ILP has been demonstrated.
In this paper, we partially address these shortcomings by examining the construction of discriminatory
problems defined over Bongard-like problems \cite{bongard}. As in the chess-endgame approach considered
by Quinlan, it is possible to pose increasingly difficult discrimination tasks based on complex
geometric concepts. Using a selection of such problems, categorised roughly of low-, medium- and
high-complexity we develop a method for automatically extracting higher-level representations of the
data as the result of computation by the program synthesised. Using Dreamcoder
and a well-known ILP engine (Aleph: \cite{aleph}) we provide evidence supporting the claim
that if neural-program synthesis can find a generative program, then ILP can construct a discriminative
model using abstractions extracted automatically from the program's computation. We also find
there are high-complexity Bongard problems for which neural-based program synthesis fails, and
identify possible reasons for this. 

The rest of the paper is organised as follows.
	


==> intro_gs.tex <==
Quoting from [Mellanie Mitchell AI], `` `Forming abstractions’ was one of the key AI 
abilities listed in the 1955 Dartmouth AI proposal’’, and ``However, enabling machines to form humanlike conceptual abstractions is still an almost completely unsolved problem.’’
In 1967 Mikhail Bongard proposed [ ] a set of 100 puzzles
designed so as to challenge the abstraction and analogy-making abilities
of both humans and AI systems. 

Each Bongard problem captures a unique abstract concept in the space of drawings
of shapes and lines, along with six positive examples and six negative ones. For
example, the concept could be `same shapes’ in which all the shapes in a positive
example are the same, e.g., all squares, or all triangles, whereas a negative example
might contain different shapes. The puzzle is to guess whether a new drawing is positive
or negative, i.e., a standard classification problem. However, the new drawing may
not contain \it{any} of the shapes present in the training examples, e.g., it may
contain all circles vs circles and pentagons. So, recognising shapes from
amongst those seen in the twelve training drawings alone would not be sufficient
to classify a drawing. Instead, the higher-level abstraction of ‘sameness’ would need
to be learned.

Further, an important feature of Bongard problems is that they each require very different 
concepts to solve, and so challenge the solvers ability to create new and high-level abstractions
‘on the fly’ from very few examples. As a consequence, a human learner would be unlikely to glean
any greater insight from having solved many Bongard problems vs having merely seen many drawings
and `understood’ them.

Since the concepts required for each Bongard puzzle are different, an AI
system for solving Bongard problems would need to form the required abstractions rapidly (i.e.,
from very few examples) using simpler ones that are both sufficiently powerful as well 
as problem-specific. Further, there are only a hundred or so Bongard problems, so a 
data-intensive approach that assumes access to large volumes of similar problems is ruled out. 

Of course, drawings of shapes and lines as in Bongard problems are by themselves not in 
short supply. One could conceivably learn features from a large number of such drawings
in an self-supervised manner, e.g., using deep learning. Exactly such an approach was
used in [ ]. However, quoting [ ] once more: ``The trained ConvNets performed only slightly better than random guessing on these “same versus different” problems, whereas the humans tested by the authors scored close to 100 percent.’’ and ``In short, today’s ConvNets, . . . do not have what it takes to do the kinds of abstraction and analogy making required even in Bongard’s idealized problems’’.

Thus the question arises as to what kind of high-level features might suffice to enable
rapid analogy-making, i.e., capturing the `essential’ similarity between one set of drawings
vs another.

The `Dreamcoder’ program induction procedure [Dreamcoder] synthesizes a \it{program} to solve 
problems. In particular, given a drawing such as those involved in Bongard puzzles, it produces
a program to re-draw it. Further, as shown in [Dreamcoder], as the system generates more
programs, it analyses them to find opportunities to re-factor code into higher-level procedures
that are, in turn, used to generate shorter programs for future problems. Thus, while starting
from very simple primitives, such as `move forward’, `turn left’, `pen up/down’, etc., Dreamcoder
would \it{abduce} new functions to `draw a triangle’ for instance; of course, the the function
produced would not refer to the term `triangle’, it might call it `f12’, for example.

We postulate that the programs that re-draw the drawings in a Bongard puzzle should serve
as good intermediate abstractions from which to learn, `on the fly’, the concept involved.
For examples, if the concept were `sameness’, programs that generated positive drawings
would not contain different high-level functions, instead the same function would occur 
repeatedly. 

Further, we suggest that inductive logic programming (ILP) can be used to learn a
first-order-logic(FOL) theory over the set of programs generating positive and negative drawings, 
and this theory would embody the concept involved in the particular Bongard puzzle in question.
A new drawing could them be classified by first generating the program to re-draw it,
using Dreamcoder, and then applying the above FOL-theory on the generated program.

<Outline: …>









 

 

==> tables/dreamcoder-hyperparameters.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|c|c|}
\hline
Hyperparameter & Value \\ \hline
\begin{tabular}[c]{@{}c@{}}Enumeration\\ Timeout\end{tabular} & 7200 \\ \hline
TopK & 1 \\ \hline
CPU cores & 8 \\ \hline
Arity & 3 \\ \hline
Maximum Frontiers & 10 \\ \hline
\begin{tabular}[c]{@{}c@{}}Recognition Model\\ Training Timeout\end{tabular} & 3600 \\ \hline
Bias Optimality & True \\ \hline
Pseudo Counts & 30 \\ \hline
aic & 1.0 \\ \hline
Structure Penalty & 1.5 \\ \hline
\end{tabular}%}
\caption{Dreamcoder Hyperparameters}
\label{tab:dreamcoder-hyperparams}%}
\end{table*}

==> tables/dreamcoder-hyperparams-and-primitives.tex <==
\begin{table*}[]
\centering
\begin{adjustbox}{width=0.6\linewidth}
\begin{tabular}{|c|c|}
\hline
Primitive & Description \\ \hline
1, 2, ..., 9 & Integers from  1 to 9 \\ \hline

\verb|ifty| & Integer 20 \\ \hline

\verb|ul|, \verb|ua| & Unit length and angle.\\ \hline

\verb|epsl|, \verb|epsa| & Epsilon length and angle.\\ \hline

\begin{tabular}[c]{@{}c@{}}\verb|mull|, \verb|div|, \\\verb|add|, \verb|sub|\end{tabular} & 

\begin{tabular}[c]{@{}c@{}}Basic arithmetic operations \\for angles and lengths\end{tabular}                                 \\ \hline

\verb|fwrtinteps| & \begin{tabular}[c]{@{}c@{}}Given two integers x and y:\\ moves forward by 0.05 * x and \\ rotates by 0.025 * y\end{tabular} \\ \hline
\verb|rtfwint| & \begin{tabular}[c]{@{}c@{}}Given two integers x and y:  \\ rotates by (2 pi / y) and \\ moves forward by 1 * x\end{tabular} \\ \hline
\verb|loop| & \begin{tabular}[c]{@{}c@{}}Given an integer x and a program p:\\ loops x times and executes p each time\end{tabular} \\ \hline
\verb|pt| & \begin{tabular}[c]{@{}c@{}}Given a program p:\\ Pen-up, executes p, pen down\end{tabular} \\ \hline
\end{tabular}
\end{adjustbox}
\quad
\centering
\begin{tabular}{|c|c|}
\hline
Hyperparameter & Value \\ \hline
\begin{tabular}[c]{@{}c@{}}Enumeration\\ Timeout\end{tabular} & 7200 \\ \hline
TopK & 1 \\ \hline
CPU cores & 8 \\ \hline
Arity & 3 \\ \hline
Maximum Frontiers & 10 \\ \hline
\begin{tabular}[c]{@{}c@{}}Recognition Model\\ Training Timeout\end{tabular} & 3600 \\ \hline
Bias Optimality & True \\ \hline
Pseudo Counts & 30 \\ \hline
aic & 1.0 \\ \hline
Structure Penalty & 1.5 \\ \hline
\end{tabular}%}
\caption{Dreamcoder Primitives and Hyperparameters}
\label{tab:dreamcoder-hyperparams-and-primitives}%}
\end{table*}

==> tables/dreamcoder-primitives.tex <==
\begin{table*}[]
\centering
\begin{adjustbox}{width=0.6\linewidth}
\begin{tabular}{|c|c|}
\hline
Primitive & Description \\ \hline
1, 2, ..., 9 & Integers from  1 to 9 \\ \hline

\verb|ifty| & Integer 20 \\ \hline

\verb|ul|, \verb|ua| & Unit length and angle.\\ \hline

\verb|epsl|, \verb|epsa| & Epsilon length and angle.\\ \hline

\begin{tabular}[c]{@{}c@{}}\verb|mull|, \verb|div|, \\\verb|add|, \verb|sub|\end{tabular} & 

\begin{tabular}[c]{@{}c@{}}Basic arithmetic operations \\for angles and lengths\end{tabular}                                 \\ \hline

\verb|fwrtinteps| & \begin{tabular}[c]{@{}c@{}}Given two integers x and y:\\ moves forward by 0.05 * x and \\ rotates by 0.025 * y\end{tabular} \\ \hline
\verb|rtfwint| & \begin{tabular}[c]{@{}c@{}}Given two integers x and y:  \\ rotates by (2 pi / y) and \\ moves forward by 1 * x\end{tabular} \\ \hline
\verb|loop| & \begin{tabular}[c]{@{}c@{}}Given an integer x and a program p:\\ loops x times and executes p each time\end{tabular} \\ \hline
\verb|pt| & \begin{tabular}[c]{@{}c@{}}Given a program p:\\ Pen-up, executes p, pen down\end{tabular} \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Dreamcoder Primitives}
\label{tab:dreamcoder-primitives}
\end{table*}

==> tables/old.tex <==

% \begin{table}[!h]
% \centering
% \resizebox{\columnwidth}{!}{
% \renewcommand*{\arraystretch}{1.5}
% \begin{tabular}{||c|c|c|c||}
% \hline
% \textbf{BP \#} & \textbf{Concept} & \textbf{Library}  & \textbf{Theory} \\ \hline \hline
% BP 4 & Concavity &  &  \\ \hline
% BP 16 & Clockwise & & \begin{tabular}[c]{@{}c@{}}\textbf{pos(A)} :- has\_info(A,B,f4,{[}D,E,F{]}).\\ \textbf{pos(A)} :- has\_info(A,B,f6,{[}D,E,F{]}).\end{tabular} \\ \hline
% BP 21 & Smaller Shape present &  &  \\ \hline
% BP 23 & Number of Shapes & & \begin{tabular}[c]{@{}c@{}}\textbf{pos(A)} :- trace(A,B), \\ B={[}C \textpipe D{]}, D={[}E \textpipe F{]}, F={[}{]}.\end{tabular}  \\ \hline
% BP 24 & Circle present & & \textbf{pos(A)} :- has\_info(A,B,f0,D,{[}E,F,G{]}).  \\ \hline
% BP 36 & Triangle above Square & & \begin{tabular}[c]{@{}c@{}}\textbf{pos(A)} :-\\    has\_info(A,B,f3,{[}C,D,E{]}), \\ has\_info(A,B,f1,{[}F,G,H{]}), G \textgreater{} D.\end{tabular} \\ \hline
% BP 40 & Collinearity &  &  \\ \hline
% BP 53 & Inside / Outside &  &  \\ \hline
% BP 60 & Two Similar Shapes & & \begin{tabular}[c]{@{}c@{}}\textbf{pos(A)} :- has\_info(A,B,C,D,{[}E,F,G{]}),\\  has\_info(A,H,C,I,{[}J,K,L{]}), H\textbackslash{}==B.\end{tabular} \\ \hline
% BP 75 & \begin{tabular}[c]{@{}c@{}}Triangle on Concave \\ side of Arc\end{tabular} & & \begin{tabular}[c]{@{}c@{}}\textbf{pos(A)} :- has\_info(A,B,f0,C,{[}D,E,F{]}), \\ bw\_90\_270(F), \\ has\_info(A, G, f1, H, {[}I, J, K{]}), D\textgreater{}I. \\ \textbf{pos(A)} :- has\_info(A,B,f0,C,{[}D,E,F{]}), \\ has\_info(A, G, f1, H, {[}I, J, F{]}), \\ bw\_270\_90(K), I\textgreater{}D.\end{tabular} \\ \hline
% \end{tabular}}
% \\
% \caption{Final Theory Learnt by our System}
% \label{tab:result-theories}
% \end{table}



%BP16: pos(A) :- has_info(A,B,f4,[D,E,F]).
%      pos(A) :- has_info(A,B,f6,[D,E,F]).
%BP21: pos(A) :-
%   has_info(A,B,rtfwint,C,[D,E,F]), C=[G|H], H=[I|J], G>I,
%   has_info(A,K,f1,L,[D,E,F]).
%pos(A) :-  has_info(A,B,f1,C,[D,E,F]), C=[G|H], H=[I|J], G>I.
%BP36: pos(A) :- has_info(A,B,f3,[C,D,E]), has_info(A,B,f1[F,G,H]), G>D.
%BP23: pos(A) :- trace(A,B), B=[C|D], D=[E|F], F=[].
%BP24: pos(A) :- has_info(A,B,f0,D,[E,F,G]).
%BP60: pos(A) :- has_info(A,B,C,D,[E,F,G]), has_info(A,H,C,I,[J,K,L]), H\==B.
%BP75: pos(A) :- has_info(A,B,f0,C,[D,E,F]), bw_90_270(F), has_info(A, G, f1, H, [I, J, K]), D>I.
%      pos(A) :- has_info(A,B,f0,C,[D,E,F]), has_info(A, G, f1, H, [I, J, F]), bw_270_90(), I>D.

==> tables/old_pos.tex <==


% \begin{adjustbox}{
    % addcode=
        % {\begin{minipage}{\width}}
        % {\caption{Final Theory Learnt by our System}\label{fig:result-pos-theories}\end{minipage}},
        % center, float=table}
% \begin{table*}
\begin{table}[!htbp]
\centering
\begin{adjustbox}{width=0.8\columnwidth,center}
\begin{tabular}{|l|l|l|l|} 
\hline
\textbf{Concept} & \begin{tabular}[c]{@{}l@{}}\textbf{Invented Primitives}\\\textbf{used in Theory}\end{tabular} & \textbf{Theory} & \textbf{Explanation} \\ 
\hhline{|:====:|}
 \begin{tabular}[c]{@{}l@{}}Anti-clockwise\\vs clockwise\\BP \#16\end{tabular} & \begin{tabular}[c]{@{}l@{}}\verb|f2(a0)|, \verb|f3(a0)| both~\\draw anti-clockwise spirals\\ with \verb|a0|~controlling tightness\\of the spiral. \verb|f2| uses\\step length 2 and \verb|f3|\\uses step length 1.\\\end{tabular} & \begin{tabular}[c]{@{}l@{}}\verb|pos(A) :-| \\~\verb|has_info(A,B,f3,C,[D,E,F]).|\\ \\~\verb|pos(A) :-|\\~\verb|has_info(A,B,f2,C,[D,E,F]).|\end{tabular} & \begin{tabular}[c]{@{}l@{}}Presence of invented primitive\\for drawing spirals that are\\anti-clockwise.~\end{tabular} \\ 
\hline


\begin{tabular}[c]{@{}l@{}}Smaller shape \\present\\BP \#21\end{tabular} & \begin{tabular}[c]{@{}l@{}}\verb|f1(a0, a1)|:\\Draw an \verb|a0|-sided\\polygon with\\sides of length \verb|12|\end{tabular} & \begin{tabular}[c]{@{}l@{}}\verb|pos(A) : -| \\\verb|has_info(A,B,rtfwint,C,[D,E,F]),|\\\verb+C=[G|H],H=[I|J],G>I+, \\\verb+has_info(A,K,f1,L,[D,E,F]).+\\ \\\verb|pos(A) :-| \\ \verb|has_info(A,B,f1,C,[D,E,F]),|\\\verb+C=[G|H],H=[I|J],G>I.+\end{tabular} & \begin{tabular}[c]{@{}l@{}}Either the program contains \\ a move primitive where one of\\ the arguments (division factor\\ for angle) is greater the the\\other (multiplication factor for\\ distance), or there is a polygon\\ with length of side less than \\ number of sides. Indicating \\ the shape is small.\end{tabular}  \\ 
\hline


\begin{tabular}[c]{@{}l@{}}Number of \\Shapes\\BP \#23\end{tabular} & - & \begin{tabular}[c]{@{}l@{}}\verb|pos(A)} :- trace(A,B),|\\\verb+B=[C|D], D=[E|F], F=[]+.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Contains only 2 states (in which\\ only one shape can be drawn since \\first state is always initial state).\end{tabular}\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Circle present\\BP \#24 \end{tabular} & \begin{tabular}[c]{@{}l@{}}\verb|f0(a0)|: \\Draw a~circle~with \\radius \verb|a1|.~\end{tabular} & \begin{tabular}[c]{@{}l@{}}\verb|pos(A) :-|\\\verb|has_info(A,B,f0,D,[E,F,G]).|\end{tabular} & \begin{tabular}[c]{@{}l@{}}Presence of invented primitive for drawing circle.\end{tabular}\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Triangle above \\Square\\BP \#36\end{tabular} & \begin{tabular}[c]{@{}l@{}}\verb|f1(a0)|: Draws a\\triangle of side\\length \verb|a0|.\\\\\verb|f3(a0)|: Draws a~\\square of side~\\length \verb|a0|\end{tabular} & \begin{tabular}[c]{@{}l@{}}\verb|pos(A) :-|\\ \verb|has_info(A,B,f3,C,[D,E,F]),|\\ \verb|has_info(A,G,f1,H,[I,J,K]),|\\\verb|J>E.|\end{tabular} & \begin{tabular}[c]{@{}l@{}}Triangle exists with y coordinate~\\greater than that of square.\end{tabular}\\ 
\hline

\begin{tabular}[c]{@{}l@{}}More sides\\of enclosing \\ shape\\BP \#53\end{tabular} & \begin{tabular}[c]{@{}l@{}}\verb|f1(a0, a1)|:\\Draw an \verb|a0|-sided\\polygon with\\sides of length \verb|12|\end{tabular} & 
\begin{tabular}[c]{@{}l@{}}\verb|pos(A) :-|\\
\verb|has_info(A,B,f0,C,[D,E,F]),|\\
\verb|has_info(A,R,pt,Q,[K,L,M]),|\\
\verb|has_info(A,I,f0,J,[K,L,M]),|\\
\verb+C=[G|H],J=[N|O], O=[P|Q],+\\
\verb+G>N, N>P.+
\end{tabular} & 
\begin{tabular}[c]{@{}l@{}}Smaller polygon (length of side \\ smaller than number of sides) \\ has has fewer sides than larger \\ (enclosing) polygon.\end{tabular}\\ 
\hline


%pos(A) :-
%   has_info(A,B,f0,C,[D,E,F]), C=[G|H], has_info(A,I,f0,J,[K,L,M]), J=[N|O], 
%   O=[P|Q], N>P, G>N, has_info(A,R,pt,Q,[K,L,M]).

\begin{tabular}[c]{@{}l@{}}Two Similar \\Shapes\\BP \#60\end{tabular} & - & \begin{tabular}[c]{@{}l@{}}\verb|pos(A) :- |\\\verb|has_info(A,B,C,D,[E,F,G]),|\\ \verb|has_info(A,H,C,I,[J,K,L]),|\\\verb|H\==B.|\end{tabular} & \begin{tabular}[c]{@{}l@{}}There are two shapes which are \\different (i.e. calls on two \\different invented primitives)\end{tabular}\\ 
\hline
\begin{tabular}[c]{@{}l@{}}Triangle on \\concave\\side of arc\\BP \#75\end{tabular} & \begin{tabular}[c]{@{}l@{}}\verb|f0(a0)|:\\Draws an arc of~\\radius \verb|a0|\\\\\verb|f1(a0)|: draws a\\triangle of side~\\length \verb|a0|\end{tabular} & \begin{tabular}[c]{@{}l@{}}\verb|pos(A) :-|\\ \verb|has_info(A,B,f0,C,[D,E,F]),|\\\verb|bw_90_270(F),|\\\verb|has_info(A,G,f1,H,[I,J,K]),D>I.|\\ \\\verb|pos(A) :-|\\ \verb|has_info(A,G,f1,H,[I,J,F]),|\\\verb|bw_270_90(K),I>D.|\end{tabular} & \begin{tabular}[c]{@{}l@{}}Either arc is facing right hand side \\and x coordinates of triangle is \\greater than those of arc, or arc is\\facing left and x coordinate\\of triangle is less than that of arc\end{tabular}                                                                                                                                                \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Solutions for Bongard Problems using our approach.}
\label{tab:result-pos-theories}
\end{table}
% \end{adjustbox}

==> tables/pos_neg.tex <==
\begin{table*}[!htpb]
% \resizebox{2\linewidth}{!}{
% \begin{adjustbox}{2\textwidth}
\parbox{0.25\textwidth}{
% \centering
\begin{adjustbox}{width=0.25\textwidth}
\begin{tabular*}{0.535\textwidth}{|c|c|c|} 
\hline
\textbf{Concept}                                                                        & \textbf{Failure Stage}                                   & \textbf{Explanation}                                                                        \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Concave vs\\convex\\(BP \#4)\end{tabular}                    & \begin{tabular}[c]{@{}c@{}}Representation\\\end{tabular} & \begin{tabular}[c]{@{}c@{}}Solid fills~\\cannot be~\\represented\end{tabular}      \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Large total~\\line length\\(BP\# 14)\end{tabular}            & Representation                                           & \begin{tabular}[c]{@{}c@{}}Arbitrary curves\\cannot be~\\represented\end{tabular}  \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Collinearity\\(BP \#40)\end{tabular}                         & Search                                                   & \begin{tabular}[c]{@{}c@{}}Two many\\shapes to be\\drawn\end{tabular}              \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Number of~\\Lines\\(BP\# 85)\end{tabular}                    & Search                                                   & \begin{tabular}[c]{@{}c@{}}Unable to draw\\5 irregular lines\end{tabular}          \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Location of\\solid shape\\(BP \#94)\end{tabular}             & Representation                                           & \begin{tabular}[c]{@{}c@{}}Solid fills~\\cannot be~\\represented\end{tabular}      \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Number of\\sides of\\filled in\\shape\\(BP\#96)\end{tabular} & Search                                                   & \begin{tabular}[c]{@{}c@{}}Too many lines\\to be drawn\end{tabular}                \\
\hline
\end{tabular*}
\end{adjustbox}
\caption{Examples where our system fails}
\label{tab:result-neg-theories}}
% \quad
\centering
\parbox{.6\textwidth}{
\begin{adjustbox}{width=0.6\textwidth}
\hfill
{\tiny{
\begin{tabular*}{\textwidth}{|P{1.8cm}|P{3cm}|P{3.5cm}|P{3.5cm}|}
\hline
\textbf{Concept} & \textbf{Invented Predicates Used in Theory} & \textbf{Theory} & \textbf{Explanation} \\
\hline
Anti-clockwise vs Clockwise (BP~\#16) &

    {\tt f2(a0)}, {\tt f3(a0)} both draw anti-clockwise spirals with {\tt a0} controlling tightness of the spiral. {\tt f2} uses step length 2 and {\tt f3} uses step length 1. &
    
    {\tt pos(A):- has\_info(A,B,f3,C,[D,E,F]).} 
    \textcolor{white}{\rule{10pt}{3ex}}   \hfill. %% for empty line
    {\tt pos(A):- has\_info(A,B,f2,C,[D,E,F]).} &
    Presence of invented primitive for drawing spirals that are anti-clockwise. \\ \hline
    
Smaller shape present (BP~\#21) &

    {\tt f2(a0)}, {\tt f3(a0)} both draw anti-clockwise spirals with {\tt a0} controlling tightness of the spiral. {\tt  f2} uses step length 2 and {\tt f3} uses step length 1. &
    
    {\tt pos(A) : -}
        {\tt has\_info(A,B,rtfwint,C,[D,E,F]),}
        {\tt C=[G|H],H=[I|J],G>I},
        {\tt has\_info(A,K,f1,L,[D,E,F]).} 
    \textcolor{white}{\rule{100pt}{3ex}}   \hfill
    {\tt pos(A) :-}
        {\tt has\_info(A,B,f1,C,[D,E,F]),}
        {\tt C=[G|H],H=[I|J],G>I.} & 
    
    the program contains a move primitive where the division factor for angle is greater than multiplication factor for distance, \hfill \textit{or} \hfill there is a polygon with side length less than number of sides. Indicating the shape is small. \\ 
\hline
Number of Shapes (BP~\#23) & - & 
{\tt pos(A) :- trace(A,B),} {\tt B=[C|D], D=[E|F], F=[]} 
& Contains only 2 states (in which only one shape can be drawn since first state is always initial state). \\
\hline

Circle present (BP~\#24) & 
{\tt f0(a0)}: Draw a circle with radius {\tt a1} &
{\tt pos(A) :-}  {\tt has\_info(A,B,f0,D,[E,F,G]).} & 
Presence of invented primitive for drawing circle. \\
\hline

Triangle above Square (BP~\#36) &
{\tt f1(a0)}: Draws a triangle of side length {\tt a0}. {\tt f3(a0)}: Draws a square of side length {\tt a0} &
{\tt pos(A) :-} {\tt has\_info(A,B,f3,C,[D,E,F]),} {\tt has\_info(A,G,f1,H,[I,J,K]),} {\tt J>E.}
& 
Triangle exists with y coordinate greater than that of square\\
\hline

Enclosed shape has fewer sides (BP~\#53) &
{\tt f1(a0, a1)}: Draw an {\tt a0}-sided polygon with sides of length {\tt a1} &
{\tt pos(A) :-}
{\tt has\_info(A,B,f0,C,[D,E,F]),}
{\tt has\_info(A,R,pt,Q,[K,L,M]),}
{\tt has\_info(A,I,f0,J,[K,L,M]),}
{\tt C=[G|H],J=[N|O], O=[P|Q],}
{\tt G>N, N>P.} &
Smaller polygon (length of side smaller than number of sides) has has fewer sides than larger (enclosing) polygon. \\
\hline

Two Similar Shapes (BP~\#60) & - & 
{\tt pos(A) :-} 
{\tt has\_info(A,B,C,D,[E,F,G]),} 
{\tt has\_info(A,H,C,I,[J,K,L]),}
{\tt H\==B.} & 
There are two shapes which are different (i.e. calls on two different invented primitives)  
\\
\hline

Triangle on concave side of arc (BP~\#75) & 
{\tt f0(a0)}: Draws an arc of radius {\tt a0} \hfill {\tt f1(a0)}: draws a triangle of side length {\tt a0} & 
{\tt pos(A) :-}
{\tt has\_info(A,B,f0,C,[D,E,F]),}
{\tt bw\_90\_270(F),} 
{\tt has\_info(A,G,f1,H,[I,J,K]),D>I.}
\textcolor{white}{\rule{100pt}{3ex}}   \hfill
{\tt pos(A) :-} {\tt has\_info(A,G,f1,H,[I,J,F]),}
{\tt bw\_270\_90(K),I>D.} &
Triangle exists with y coordinate greater than that of square. \\
\hline
\end{tabular*}}}
\end{adjustbox}
\caption{Solutions for Bongard Problems using our approach.}
\label{tab:result-pos-theories}}
\end{table*}

